Precise SMEFT predictions for di-Higgs production

We present results of precision calculations for di-Higgs production that combine NLO QCD corrections with operators at canonical dimension six within Standard Model Effective Field Theory (SMEFT). We discuss possible options for operator contributions within a given EFT framework and sources of theory uncertainties.

==> Makefile <==
NAME = HH_preciseSMEFT_LHCP_main
BIB = HH_preciseSMEFT_LHCP_main.bib
OTHER = $(wildcard *.tex) $(wildcard figures/*)
TEXFLAGS = --synctex=1
PYTHON = python3

ifdef PLOTS
OTHER = plots
endif

$(NAME).pdf: $(NAME).tex $(NAME).bbl $(OTHER)
	pdflatex $(TEXFLAGS) $(NAME)
	pdflatex $(TEXFLAGS) $(NAME)

$(NAME).bbl: $(NAME).tex $(BIB)
	pdflatex $(TEXFLAGS) $(NAME)
	bibtex $(NAME)

#plots/mhh.pdf: plots/mhh.py
#	cd plots && $(PYTHON) mhh.py && cd ..

clean:
	rm -rf $(NAME).pdf *.aux  *.blg *.lof *.log *.lol *.lot \
	*.out *.tcp *.toc *.tps *.synctex.gz *~ figs/*/*-converted-to*

